Automatic Verification of Message-Based Device Drivers

We develop a practical solution to the problem of automatic verification of the interface between device drivers and the OS. Our solution relies on a combination of improved driver architecture and verification tools. It supports drivers written in C and can be implemented in any existing OS, which sets it apart from previous proposals for verification-friendly drivers. Our Linux-based evaluation shows that this methodology amplifies the power of existing verification tools in detecting driver bugs, making it possible to verify properties beyond the reach of traditional techniques.

==> eptcsdata.tex <==
\providecommand{\firstpage}{4}
\providecommand{\publicationstatus}{F. Cassez, R. Huuck, G. Klein and B. Schlich (eds.):\\ Systems Software Verification Conference 2012 (SSV 2012)\\
EPTCS 102, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.102.3}{10.4204/EPTCS.102.3}}

